Mitigating Preference Leakage via Strict Estimator Separation for Normative Generative Ranking

In Generative Information Retrieval (GenIR), the bottleneck has shifted from generation to the selection of candidates, particularly for normative criteria such as cultural relevance. Current LLM-as-a-Judge evaluations often suffer from circularity and preference leakage, where overlapping supervision and evaluation models inflate performance. We address this by formalising cultural relevance as a within-query ranking task and introducing a leakage-free two-judge framework that strictly separates supervision (Judge B) from evaluation (Judge A). On a new benchmark of 33,052 (NGR-33k) culturally grounded stories, we find that while classical baselines yield only modest gains, a dense bi-encoder distilled from a Judge-B-supervised Cross-Encoder is highly effective. Although the Cross-Encoder provides a strong supervision signal for distillation, the distilled BGE-M3 model substantially outperforms it under leakage-free Judge~A evaluation. We validate our framework on the human-curated Moral Stories dataset, showing strong alignment with human norms. Our results demonstrate that rigorous evaluator separation is a prerequisite for credible GenIR evaluation, proving that subtle cultural preferences can be distilled into efficient rankers without leakage.

==> tikz-figure.tex <==
\definecolor{corpblue}{RGB}{235, 245, 255}    
\definecolor{darkblue}{RGB}{45, 85, 125}      
\definecolor{corpred}{RGB}{255, 240, 240}     
\definecolor{darkred}{RGB}{145, 45, 45}       
\definecolor{slate}{RGB}{240, 242, 245}       
\definecolor{charcoal}{RGB}{70, 75, 80}       

\begin{figure*}[t]
\centering
\resizebox{0.98\textwidth}{!}{%
\begin{tikzpicture}[
    node distance=1.2cm and 1.8cm,
    font=\sffamily,
    >={LaTeX[round]},
    line width=0.9pt,
    % Styles
    model/.style={rectangle, rounded corners=8pt, minimum width=2.5cm, minimum height=1.0cm, draw=charcoal!30, fill=white, drop shadow={opacity=0.15, shadow xshift=1pt, shadow yshift=-1pt}, font=\bfseries\footnotesize, text=charcoal, align=center},
    judge/.style={circle, minimum size=1.5cm, draw=orange!50, thick, fill=orange!5, font=\bfseries\footnotesize, text=charcoal, align=center, drop shadow={opacity=0.15}},
    op/.style={diamond, aspect=1.5, inner sep=1pt, draw=charcoal!40, fill=slate, font=\bfseries\tiny, text=charcoal, align=center},
    data/.style={rectangle, rounded corners=2pt, fill=slate, draw=none, font=\itshape\scriptsize, text=charcoal, inner sep=4pt},
    flow/.style={->, draw=charcoal!80, thick},
    grad/.style={->, draw=darkblue, dashed, thick},
    leakage/.style={draw=darkred, ultra thick, dotted},
    mathlabel/.style={fill=white, inner sep=1.5pt, rounded corners=2pt, text=charcoal, font=\tiny\scshape, draw=charcoal!10}
]
    % LEFT: GENERATION SOURCE
    \node[data, align=left] (query) {Query Constraints\\$q = (Age, Moral, Culture)$};
    \node[model, right=1.0cm of query] (generator) {Generator $G$\\$P_\phi(s|q)$};
    \node[data, right=1.0cm of generator, text width=1.8cm, align=center] (pool) {Candidate Pool\\$\mathcal{S}_q$};
    \draw[flow] (query) -- (generator);
    \draw[flow] (generator) -- (pool);
    
    % TOP STREAM: SUPERVISION LOOP
    \node[judge, above right=1.5cm and 1.5cm of pool] (judgeB) {Judge B\\(Supervisor)};
    \node[op, right=1.2cm of judgeB] (sampling) {Pairwise\\Sampling};
    \node[model, right=1.2cm of sampling, fill=corpblue, draw=darkblue!30] (ranker_train) {Ranker $f_\theta$\\Optimization};
    \node[op, right=1.2cm of ranker_train] (loss) {Loss\\$\mathcal{L}_{Rank}$};
    % Connections Top
    \draw[flow] (pool) |- (judgeB);
    \draw[flow] (judgeB) -- node[mathlabel, above] {$y_B$} (sampling);
    \draw[flow] (sampling) -- node[mathlabel, above] {$\mathcal{D}_{train}$} (ranker_train);
    \draw[flow] (ranker_train) -- (loss);
    \draw[grad] (loss.south) to[out=-150, in=-30] node[mathlabel, below] {$\nabla_\theta$} (ranker_train.south);
    
    % BOTTOM STREAM: EVALUATION LOOP
    \node[judge, below right=1.5cm and 1.5cm of pool] (judgeA) {Judge A\\(Evaluator)};
    \node[model, right=3.5cm of judgeA, fill=corpred, draw=darkred!30] (ranker_test) {Ranker $f_{\theta^*}$\\Inference};
    \node[op, right=1.2cm of ranker_test] (metric) {Metric\\nDCG@k};
    % Connections Bottom
    \draw[flow] (pool) |- (judgeA);
    \draw[flow] (judgeA) to[out=0, in=-130] node[mathlabel, below, near end] {$y_A$ (Ground Truth)} (metric);
    \draw[flow] (ranker_test) -- node[mathlabel, above] {$\hat{y}$} (metric);
    \draw[flow] (pool) to[out=-30, in=210] (ranker_test.west);
    
    % TRANSFER
    \draw[->, ultra thick, darkblue, densely dashed] (ranker_train.south) -- ++(0,-1.0) -| (ranker_test.north) node[pos=0.25, right, font=\bfseries\tiny, text=darkblue, fill=white, inner sep=2pt] {Parameter Transfer $\theta^*$};
    
    % BARRIER (Creatively Adjusted)
    % We define the vertical midpoint
    \coordinate (mid_v) at ($(judgeB.south)!0.5!(judgeA.north)$);
    % Start the line specifically to the RIGHT of the pool to avoid text overlap
    \draw[leakage] ($(pool.east |- mid_v) + (0.5, 0)$) -- ($(metric.east |- mid_v) + (0.5, 0)$);
    % Center the label on this new shorter line
    \node[fill=white, text=darkred, font=\bfseries\tiny, draw=darkred!20, rounded corners, inner sep=3pt] at (sampling |- mid_v) {STRICT INFORMATION BARRIER (STOP GRADIENT)};
    
    % BACKGROUND ZONES
    \begin{scope}[on background layer]
        \node[fit=(judgeB) (loss) (ranker_train), fill=corpblue, rounded corners=12pt, inner sep=10pt] (zone_top) {};
        \node[above left, text=darkblue, font=\bfseries\large, yshift=-5pt] at (zone_top.north west) {Phase I: Supervision (Offline)};
        \node[fit=(judgeA) (metric) (ranker_test), fill=corpred, rounded corners=12pt, inner sep=10pt] (zone_bot) {};
        \node[below left, text=darkred, font=\bfseries\large, yshift=5pt] at (zone_bot.south west) {Phase II: Evaluation (Online)};
    \end{scope}
\end{tikzpicture}%
}
\caption{The Leakage-Free Ranking Framework. We rigorously separate the optimisation loop (Top, Blue) from the inference/evaluation loop (Bottom, Red). The Supervision Judge ($J_B$) generates noisy proxies $y_B$ for gradient descent ($\nabla_\theta$). The Independent Evaluator ($J_A$) provides labels $y_A$ exclusively for metric computation. The only bridge between the worlds is the frozen parameter set $\theta^*$, preventing circular preference leakage.}
\label{fig:framework_sophisticated}
\end{figure*}
